The Power of Greedy for Online Minimum Cost Matching on the Line

We consider the online minimum cost matching problem on the line, in which there are $n$ servers and, at each of $n$ time steps, a request arrives and must be irrevocably matched to a server that has not yet been matched to, with the goal of minimizing the sum of the distances between the matched pairs. Despite achieving a worst-case competitive ratio that is exponential in $n$, the simple greedy algorithm, which matches each request to its nearest available free server, performs very well in practice. A major question is thus to explain greedy's strong empirical performance. In this paper, we aim to understand the performance of greedy over instances that are at least partially random. When both the requests and the servers are drawn uniformly and independently from $[0,1]$, we show that greedy is constant competitive, which improves over the previously best-known $O(\sqrt{n})$ bound. We extend this constant competitive ratio to a setting with a linear excess of servers, which improves over the previously best-known $O(\log^3{n})$ bound. We moreover show that in the semi-random model where the requests are still drawn uniformly and independently but where the servers are chosen adversarially, greedy achieves an $O(\log{n})$ competitive ratio. When the requests arrive in a random order but are chosen adversarially, it was previously known that greedy is $O(n)$-competitive. Even though this one-sided randomness allows a large improvement in greedy's competitive ratio compared to the model where requests are adversarial and arrive in a random order, we show that it is not sufficient to obtain a constant competitive ratio by giving a tight $\Omega(\log{n})$ lower bound. These results invite further investigation about how much randomness is necessary and sufficient to obtain strong theoretical guarantees for the greedy algorithm for online minimum cost matching, on the line and beyond.

==> old_bib.tex <==
@misc{Lyft,
  title = {Matchmaking in {L}yft {L}ine},
  howpublished = {\url{https://tinyurl.com/3sdrw7yc}},
  note = {Accessed: July 10, 2022}
}

@misc{HowMatch,
  title = {How the Matching Algorithm works in the On-Demand Economy? Part Three of the User Journey Series},
  howpublished = {\url{https://jungleworks.com/matching-algorithm-works-demand-economy-part-three-user-journey-series/#:~:text=Buyer%20Pick%20Model%20%E2%80%93%20Buyer%20fills,one%20who%20accepts%20the%20request.}},
  note = {Accessed: July 10, 2022}
}

@misc{Uber,
  title = {How does {U}ber match riders with drivers?
},
  howpublished = {\url{https://www.uber.com/us/en/marketplace/matching/}},
  note = {Accessed: July 10, 2022}
}

@misc{UberEats,
  title = {How {U}ber {E}ats Uses Machine Learning to Estimate Delivery Times?},
  howpublished = {\url{https://thenewstack.io/how-uber-eats-uses-machine-learning-to-estimate-delivery-times/#:~:text=Prior%20to%20ML%2C%20Uber%20Eats,the%20drivers%20in%20that%20area.}},
  note = {Accessed: July 10, 2022}
}

@misc{UberDrivers,
  title = {Uber drivers are reportedly colluding to trigger 'surge' prices because they say the company is not paying them enough
},
  howpublished = {\url{https://www.businessinsider.com/uber-drivers-artificially-triggering-surge-prices-reports-abc7-2019-6}},
  note = {Accessed: July 14, 2022}
}


% @misc{Lyft,
%   title = {Matchmaking in {L}yft {L}ine},
%  URL = {\url{https://tinyurl.com/3sdrw7yc}},
% }

% @misc{HowMatch,
%   title = {How the Matching Algorithm works in the On-Demand Economy? Part Three of the User Journey Series},
%   URL = {\url{https://jungleworks.com/matching-algorithm-works-demand-economy-part-three-user-journey-series/#:~:text=Buyer%20Pick%20Model%20%E2%80%93%20Buyer%20fills,one%20who%20accepts%20the%20request.}},
% }

% @misc{Uber,
%   title = {How does {U}ber match riders with drivers?
% },
%   URL = {\url{https://www.uber.com/us/en/marketplace/matching/}},
%   note = {Accessed: July 10, 2022}
% }

% @misc{UberEats,
%   title = {How {U}ber {E}ats Uses Machine Learning to Estimate Delivery Times?},
%   URL = {\url{https://thenewstack.io/how-uber-eats-uses-machine-learning-to-estimate-delivery-times/#:~:text=Prior%20to%20ML%2C%20Uber%20Eats,the%20drivers%20in%20that%20area.}},
% }

% @misc{UberDrivers,
%   title = {Uber drivers are reportedly colluding to trigger 'surge' prices because they say the company is not paying them enough
% },
%   URL = {\url{https://www.businessinsider.com/uber-drivers-artificially-triggering-surge-prices-reports-abc7-2019-6}},
% }


@article{Lyft,
 author  = {Brown, Timothy},
 year    = {2016},
 title   = {Matchmaking in Lyft Line — Part 1},
 journal = {Lyft Engineering},
 url     = {https://tinyurl.com/3sdrw7yc},
 urldate = {July 10, 2022}
}

